On optimal multiplexing of an ensemble of discrete-time constrained control systems on matrix Lie groups

We study a constrained optimal control problem for an ensemble of control systems. Each sub-system (or plant) evolves on a matrix Lie group, and must satisfy given state and control action constraints pointwise in time. In addition, certain multiplexing requirement is imposed: the controller must be shared between the plants in the sense that at any time instant the control signal may be sent to only one plant. We provide first-order necessary conditions for optimality in the form of suitable Pontryagin maximum principle in this problem. Detailed numerical experiments are presented for a system of two satellites performing energy optimal maneuvers under the preceding family of constraints.

==> Conclusion.tex <==
% Conclusions
We present the first order necessary conditions of optimality for the discrete time constrained optimal control problem for systems evolving on matrix Lie groups. We consider constraints on the state and the control action trajectories. In addition to that, the controller is employed in a multiplexed fashion in the sense that at any instant the control action is provided to only one plant in the system. We validate the necessary conditions of optimality with the numerical results obtained, using a third party NLP solver (\textsf{CasADi}), for a system of two satellites performing single-axis maneuvers. 

==> Corollary.tex <==
%This provides proof of corollary
Corollary \ref{Corollary1} presents the first order necessary conditions for point-to-point reachability maneuvers of NCSs with state, action and multiplexing constraints. Proof of this follows from the ideas presented in Section \ref{sec: Proof} and the proof of \cite[Corollary 8]{phogat2016discrete}. Just to mention the approach: Proof follows by extending Theorem \ref{th: 1} to problem where final states are constrained to lie on a manifold $\mathcal{M}_{fin}$. This idea can be formalized by representing the boundary constraints $(q_N, x_N) \in \mathcal{M}_{fin}$ as state inequality constraint as presented in proof of \cite[Corollary 8]{phogat2016discrete}. Point to point reachability maneuver is then just a special case to that. 
